XpulpNN: Enabling Energy Efficient and Flexible Inference of Quantized Neural Network on RISC-V based IoT End Nodes

This work introduces lightweight extensions to the RISC-V ISA to boost the efficiency of heavily Quantized Neural Network (QNN) inference on microcontroller-class cores. By extending the ISA with nibble (4-bit) and crumb (2-bit) SIMD instructions, we are able to show near-linear speedup with respect to higher precision integer computation on the key kernels for QNN computation. Also, we propose a custom execution paradigm for SIMD sum-of-dot-product operations, which consists of fusing a dot product with a load operation, with an up to 1.64x peak MAC/cycle improvement compared to a standard execution scenario. To further push the efficiency, we integrate the RISC-V extended core in a parallel cluster of 8 processors, with near-linear improvement with respect to a single core architecture. To evaluate the proposed extensions, we fully implement the cluster of processors in GF22FDX technology. QNN convolution kernels on a parallel cluster implementing the proposed extension run 6 x and 8 x faster when considering 4- and 2-bit data operands, respectively, compared to a baseline processing cluster only supporting 8-bit SIMD instructions. With a peak of 2.22 TOPs/s/W, the proposed solution achieves efficiency levels comparable with dedicated DNN inference accelerators, and up to three orders of magnitude better than state-of-the-art ARM Cortex-M based microcontroller systems such as the low-end STM32L4 MCU and the high-end STM32H7 MCU.

==> text/04_body.tex <==
\section{Domain Specific RISC-V ISA Extension}
\subsection{\textit{XpulpNN} ISA Extension} 
\label{sec:ISA}
The RISC-V ISA we assume as our baseline, namely \textit{XpulpV2}, targets efficient digital signal processing and it exploits the SIMD computing paradigm for 16- and 8-bit vector operands, providing instructions in three addressing variations. The first uses two vector registers as source operands (\textit{pv.instr.\{b,h\}}), the second variation uses one vector register and one immediate as source operands  (\textit{pv.instr.sci.\{b,h\}}), while the last one uses one vector register and replicates the scalar value in a register as the second operand for the SIMD operation (\textit{pv.instr.sc.\{b,h\}}).
%
\begin{table}[t]
    \centering
        %\caption{Overview of \textit{XpulpNN} instructions for \textit{nibble} (4-bit) and \textit{crumb} (2-bit) vector operations. The description is provided for \textit{nibble} operations, and it can be extended to \textit{crumb}.}%\tablefootnote{(.sc) indicates the scalar replication mode, i.e. rs1 is treated as vector wile rs2 is treated as scalar and replicated eight or sixteen times to form a complete vector.}}  
        \caption{Overview of \textit{XpulpNN} instructions for \textit{nibble} (4-bit) vecotr operands. The description can be extended to \textit{crumb} (2-bit). $i$ in the table refers to the index in the vector operand, i.e. $i \in [0; 7]$ in the \textit{nibble} case. }
 
    \label{tab:xpulpnnisa}
    \begin{tabular}{l|l}
         %\multicolumn{3}{c}{\textbf{\textit{XpulpNN} \textit{nibble} (4-bit) and \textit{crumb} (2-bit) SIMD instructions}} \\
         \hline %\\
        \textbf{ALU SIMD Op.} & \textbf{Description for \textit{nibble}} \\
         pv.add[.sc].\{n, c\} &  rD[i] = rs1[i] + rs2[i]\\
          pv.sub[.sc].\{n, c\} & rD[i] = rs1[i] - rs2[i] \\ 
          pv.avg(u)[.sc].\{n, c\} & rD[i] = (rs1[i] + rs2[i])$>>$1\\
          \hline
          \textbf{Vector Comparison Op.}& \\
          pv.max(u)[.sc].\{n, c\} & rD[i] = rs1[i] $>$ rs2[i] ? rs1[i] : rs2[i]\\
          pv.min(u)[.sc].\{n, c\}& rD[i] = rs1[i] $<$ rs2[i] ? rs1[i] : rs2[i]\\ 
          \hline
          \textbf{Vector Shift Op.} & \\
          pv.srl[.sc].\{n, c\} &  rD[i] = rs1[i] $>>$ rs2[i] Shift is logical \\
          pv.sra[.sc].\{n, c\} & rD[i] = rs1[i] $>>$ rs2[i] Shift is arithmetic\\
          pv.sll[.sc].\{n, c\}& rD[i] = rs1[i] $<<$ rs2[i]\\ %& & \\
          \hline
          \textbf{Vector abs Op.} & \\
          pv.abs.\{n, c\}& rD[i] = rs1[i] $<$ 0 ? -rs1[i] : rs1[i]\\ % & & \\
          \hline
          \textbf{Dot Product Op.}& \\
          pv.dotup[.sc].\{n, c\}& rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7]\\
          pv.dotusp[.sc].\{n, c\} & rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7]\\
          pv.dotsp[.sc].\{n, c\} & rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7]\\
          pv.sdotup[.sc].\{n, c\} & rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7] + rD\\
          pv.sdotusp[.sc].\{n, c\}& rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7] + rD\\
          pv.sdotsp[.sc].\{n, c\} &  rD = rs1[0]*rs2[0] + ... + rs1[7]*rs2[7] + rD\\% & & \\
          \hline
    \end{tabular}
\end{table}

The proposed \textit{XpulpNN} instructions, listed in Table~\ref{tab:xpulpnnisa}, extend the RV32IMCXpulpV2 ISA with SIMD operations also for 4-bit and 2-bit operands, namely \textit{nibble} (indicated with \textit{n}) and \textit{\textit{crumb}} (indicated as \textit{c}) respectively, to improve the efficiency of low-bitwidth QNN kernels.
%
Because of the limited room in the encoding space of the baseline ISA, we propose the crumb and nibble operations only in two addressing variations.
% 
We do not implement the instruction format which uses an immediate value as second operand (i.e. \textit{pv.instr.sci.\{b,h\}}). 
%
Based on our experience, we argue that this choice is not a concern for the execution of QNN kernels: an immediate value can be prevently stored into a register withouth compromising the efficiency of the computation (no additional overhead).
%
The core of the \textit{Xpulpnn} ISA extension consists of the \textit{dot product} based instructions performed in a SIMD-like manner on packed vectors of 4-, 2-bit elements. 
%
The packed input registers can be interpreted as signed or unsigned, or the first signed and the second unsigned. The accumulator, as well as the third scalar input in the sum-of-dot-product, is a 32-bit signed register anytime one of the input operands is signed, while it is interpreted as unsigned in the remaining case.
%
In addition to the \textit{dot product} based operations we support also SIMD instructions like maximum, minimum and average for nibble and crumb packed operands, useful to speed-up the pooling layers and the activation layers based on the Rectified Linear Unit (ReLu) function.
%
A group of ALU based operations (addition, subtraction, shift) completes the set of the \textit{XpulpNN} SIMD arithmetic instructions.

To further speed-up the QNN convolution kernels, especially the \textit{MatMul} of the PULP-NN library, we extend the \textit{XpulpNN} ISA with a set of Mac\&Load SIMD instructions.
%
Each time we want to perform a MAC operation or a SIMD \textit{dot product} instruction on a RISC based in-order single-issue processor, we first need to bring into the Register File (RF) the two operands involved in the computation, which costs two load operations.
%
Hence we would spend three operations to perform a MAC. To ease the discussion in the following, let us define the previous concept as the efficiency of the target ISA to execute the MACs, which will result equal to $0.33$. We want this number as high as possible, known that it can not be higher than one. 
%

If in the computing kernel we exploit data reuse at the RF level, i.e. we reuse some registers as inputs of more MAC operations, we can increase the efficiency of the MAC.
%
The innermost loop of the PULP-NN \textit{MatMul} kernel performs eight SIMD \textit{sdotp} operations. Thanks to the reuse of the same \textit{im2col} elements over more filter elements at the Register File level, the \textit{sdotp}s cost six load operations, bringing the efficiency of computing the SIMD MACs to $0.57$.
%
Due to the limited number of registers (32) in the General Purpose Register File (RF) of the target architecture, the data reuse can not be increased further[cite PNN].
%
%
\begin{figure}[t]
    \centering
    \includegraphics[width= \linewidth]{images/ML_encoding.pdf}
    \caption{The figure shows: (a) the baseline assembly code of the 8-bit \textit{MatMul} kernel innermost loop of PULP-NN; (b) the prototype and the encoding of the mac\&load (\textit{ml}) instruction; (c) an enhanced version, more flexible and efficient, of the mac\&load instruction, namely ``m\&lv2''.}
    \label{fig:ml_encoding}
\end{figure}
%

Looking at the assembly code of the \textit{MatMul} kernel in Figure \ref{fig:ml_encoding}.(a) we notice that most of the loads are implemented through the post incremented load instructions, meaning that the memory access pattern of the kernel is extremely regular, being a \textit{MatMul}.
%
The first design of the Mac\&Load instruction exploits the regular pattern of the loads to improve the efficiency as follows. Anytime we have regular kernels of the type mentioned above, one of the two operands of the SIMD operation (let assume the weights, in this case) will be stored in a dedicated Special Purpose Register, namely Neural Network Register File (NN-RF), that we can dimension depending on our needs and constraints, instead of the common RF.
%
Let then provide the NN-RF with an instruction that controls its registers both as inputs for the MAC operations and as outputs for the post-incremented load.
%
Assuming the features explained above, we can store the weights into the NN-RF with a ``special'' post-increment load and fetch one of the operands for the MAC with a ``special'' sdotp and we can do it in a single fused instruction. After the initialization of the registers, the SIMD MAC unit would fetch the weight operands from a register of the NN-RF and the LOAD unit will update that register (after it is used in the current \textit{dotp-based} operation) with a new data from the memory.
%

Let consider the mac\&load encoding proposed in Figure \ref{fig:ml_encoding}.(a). The source operands of the instruction contain the second operand of the MAC while \textit{rs1} contains the address for the next memory access (to update the NN-RF). The ``SPR[i]" field specifies which register of the SPR to use as input for the MAC operation and as output of the load, where $0 \leq i \leq 3 $ having the NN-RF of size 4. The size of the NN-RF has been chosen in order to maximize the number of free registers to host all the weight operands of a single run of the \textit{MatMul }innermost loop.
%
Using the mac\&load the innermost loop of the \textit{MatMul} kernel of the PULP-NN library will look like the one in Figure \ref{fig:ml_assembly}.(a). We reduce the costs of explicit load operations to 2 to perform 8 SIMD MAC with a resulting operation efficiency of $0.8$.
%

Despite we are able to improve the efficiency of the MAC operation in the \textit{MatMul} kernel, the mac\&load proposed above has some structural limitations. First, at each call of the mac\&load instruction we are forced to always update the register currently used in the MAC operation. This is not a concern from a functional point of view since we are always able to mask all non-necessary loads into the fused instruction. However the load operations are actually performed by the Load unit of the core, causing energy-expansive accesses to the memory and interconnect, hence creating unnecessary performance degrading contentions in the context of tightly coupled shared memory clusters. 
%
Besides, only one operand will be fetched from the NN-RF. This limits the exploration of bigger \textit{MatMul} layout, since many registers of the RF are still used to store the \textit{dotp} operands.



%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/ML_assembly.pdf}
    \caption{The figure shows (a) the implementation of the 8/bit \textit{MatMul} innermost loop using the m\&lv1 instruction. Only two explicit loads are needed to execute 8 SIMD dotp operations; (b) the implementation of the innermost loop of the 8-bit \textit{MatMul} kernel using the mac\&lv2 instruction. In this case we pay only one load to execute 8 SIMD dotp operations. }
    \label{fig:ml_assembly}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/ML_4x4structure.pdf}
    \caption{The figure shows how the m\&lv2 can be used to implement bigger layout structures of the \textit{MatMul}. In particular (a) shows the classical 4$\times$2 layout with the m\&lv2. Notice that many registers of the RF are free and can be used to store more accumulators. (b) shows that by reusing more activations over more weights we can implement a 4$\times$4 layout for the \textit{MatMul} innermost loop, thanks to the m\&lv2.}
    \label{fig:ml_4x4structure}
\end{figure}

We overcome these inherent limitations by proposing a second enhanced version of the mac\&load, namely ``m\&lv2'', more flexible and efficient with respect to the previous one.
%
We change the encoding type of the instruction, using a custom instruction format introduced in the \textit{XpulpV2} ISA extension, with a single source register, the destination one and a 5-bit Immediate. 
%
The Immediate will allow us to improve the flexibility of the instruction exposing the registers of the NN-RF to be fully controlled with load, dotp, and mac\&load operations. The Figure \ref{fig:ml_encoding}.(b) shows the proposed encoding.
%
In current ``v2'' version we assume that the NN-RF consists of two regions, one dedicated to weights (consisting of 4 registers) and one to the activations (2 registers). 
%The capacity of the NN-RF, following the same reasoning as above, has been chosen to maximize the capacity of the NN-RF 
%
Since we dedicate part of the NN-RF to the weights and part to the activations, we can specialize the \textit{dotp} instruction to fetch both the operands of the MAC from the NN-RF. 
%
In this way, the RF registers will be used only to store the accumulators, leaving more room for \textit{MatMul} structure explorations.
%
More in detail, the three least significant bits of the Immediate have the functionality to address the specific NN-RF registers, one for the weights and one for the activations, as visible in Figure \ref{fig:ml_encoding}.
%
The registers selected will feed the MAC unit that will perform the operation specified by the ``OPCODE'', interpreting the registers as signed or unsigned depending on the most significant bits of the instructions and the ones that specify the data type (``DT'').
%
In the same instruction we can specify which register to update with the memory content at the address specified by ``rs1''. Since the load operation is done by the LOAD unit, we can update only one register per time in the context of one \textit{m\&lv2} instruction.

%
As will result more clearly from the Section , the ``m\&lv2'' overcomes the improvement of the ``m\&lv1'' because it allows to keep one operand into the NN-RF to be reused more time, reducing the loads pressure on the core/memory interface and it enables bigger structure of the kernel since it reduces the pressure on the RF.
%
The \textit{MatMul} kernel of the PULP-NN library, with the mac\&loadv2 is showed in Figure \ref{fig:ml_assembly}. As visible, in this case only one explicit load is needed to perform the 8 SIMD \textit{dotp} operations. Hence, the efficiency metric discussed above grows to $0.88$. At a closer look of the kernel, we notice that the number of RF registers is limited and more space is left to additional accumulators. 
%
Hence, we can fetch from the memory more \textit{im2col} elements and more weights allowing the computation of four adjacent output features of four consecutive channels (which we call ``4$\times$4 structure of the \textit{MatMul}). The assembly of such a kernel is shown in Figure \ref{fig:ml_4x4structure}. We compute 16 SIMD \textit{dotp} operations at a cost of only one explicit load, with an efficiency of $0.94$.

%
%The design of a dedicated Register File for the MAC operation (the NN-RF) alleviates the general purpose register file occupancy, now used only to store the parameters for the hardware loops and the MAC accumulators.
%
%Since any additional operand for the MAC would impact only the NN-RF occupancy and since in the GP-RF we have room to store more accumulators, we can fetch from the memory more \textit{im2col} elements and more weights allowing the computation of four adjacent output features of four consecutive channels (which we call ``4$\times$4 structure of the \textit{MatMul}). The assembly of such a kernel is shown in Figure \ref{fig:ml_4x4structure}. We compute 16 SIMD \textit{dotp} operations at a cost of only one explicit load, with an efficiency of $0.94$.

 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  COMPILER SUPPORT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Compiler Support}
\label{sec:compiler}
All the instructions of the \textit{XpulpNN} ISA extensions can be inferred in the C code by means of built-in functions. The built-ins allow the compiler to further optimize the code and the operands to get the most efficient scheduling accordingly to the underlying ISA [Beppe needed]. Moreover, the ``m\&lv2'' allows the programmer to fully control the NN-RF of the underlying hardware, even if he can not have the visibility of the variables stored in the NN-RF registers. This, of course, restricts the flexibility of the average embedded system programmer. However, our purpose is to expose the PULP-NN library functions as APIs so that the programmer never has to look at the optimized primitives to run a convolution kernel, for example. An example of this integration is in [Dory], where the backend library is integrated in a vertical QNNs deployment flow.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  MICRO-ARCHITECTURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Micro-Architecture}
\label{sec:microarchi}

% RISCY PIPELINE
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/RISCY_XpulpNN_pipe.pdf}
    \caption{The RI5CY pipeline. The Figure highlights the hardware blocks which extend the core micro-architecture to support the \textit{XpulpNN} ISA.}
    \label{fig:riscy_pipelin}
\end{figure}

%MAC UNITS
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/MAC_Units_big.pdf}
    \caption{Block diagram of the RI5CY Dot-Product Unit. To support the \textit{XpulpNN} SIMD dotp-based operations, the 8$\times$4 and the 16$\times$2 SIMD MAC Units have been added. The figure includes the clock gating blocks needed to reduce the operand switching activity.}
    \label{fig:MAC_units}
\end{figure}

% MACLOAD DATAPATH
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/ML_datapath.pdf}
    \caption{Datapath of the mac\&load instructions. The green signals/operands refer to the first implementation of the mac\&load whereas the red ones (including the additional read port of the NN-RF refer to the ``special'' mac\&load only.}
    \label{fig:ml_datapath}
\end{figure}

% OPEF SINGLE CORE
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/OPEF_1_core_allbits.pdf}
    \caption{Efficiency of the Matrix Multiplication kernel. The bar graph shows the cycles needed to the core to perform one MAC operation. The classical SIMD sdotp (XpulpNN) and the two versions of the MAC\&Load instructions (macload, nn\_custom) are considered. The nn\_custom allows also to enlarge the Matrix Multiplication layout (nn\_custom\_4x4k).}
    \label{fig:OPEF_1core}
\end{figure}



In this section we highlight the micro-architectural design to extend the baseline core (RI5CY \cite{gautschi2017near}) with the \textit{XpulpNN} ISA, focusing on the most important blocks: the dot product unit and the datapath to integrate the fused mac\&load instructions. The RI5CY pipeline and the modified blocks are reported in Figure \ref{fig:riscy_pipelin}.
%
The baseline Dot-Product Unit available in the baseline RI5CY core consists of two different sets of multipliers, one for 8-bit packed operands, the other for the 16-bit ones.
%
In the novel core we support the \textit{XpulpNN} dotp-based instructions by extending the Dot-Product unit with two additional sets of multipliers for nibble (4-bit) and crumb (2-bit) SIMD operands, as visible from Figure \ref{fig:MAC_units}.
%
The new sets of multipliers compute the dot product based operations between two SIMD registers, each containing either eight 4-bit or sixteen 2-bit elements and accumulate the partial results over a 32-bit scalar register through an adder tree, in one clock cycle of latency. 
%
The sum-of-dot-product (\textit{sdotp}) operation, which is the SIMD MAC equivalent, is supported by adding to the multipliers an additional 32-bit scalar operand at the input of each adder tree.
%
As reported in Section \ref{sec:ISA}, we support the nibble and crumb SIMD instructions interpreting the operands as signed or unsigned or first singed/ second unsigned. Hence, we provide the inputs of the SIMD multipliers with an extra-bit which sign- or zero-extends the actual single element of the SIMD vector. therefore, as depicted in Figure , each element is a 5- or 3-bit operand for the nibble and crumb cases respectively.
%

Our design choice to replicate the hardware resources to support the \textit{XpulpNN} dot-product based instructions is due to the objective of minimizing the impact of the additional hardware on the critical path of the  RI5CY core, which already involves the Dotp-Unit.
%
The nibble and crumb \textit{dotp} operations are near to be timing critical since the amount of logic to sum up all the partial products is higher than the 8- and 16-bit cases.
%
Hence, sharing the multiplication resources among all the different bitwidth "regions", or even only sharing the adder tree to sum up over all the partial multiplication contributions, would be detrimental from a timing point since the additional combinatorial logic to select, split and distribute the operands and to enable the selected bit-width SIMD operation would have a negative impact on the overall speed.
%
The main drawback of our choice is in terms of area, since we replicate hardware resources to deal with nibble and crumb operations. 
%
The power consumption of the core system would increase as well, as a direct consequence. To mitigate the effect of the hardware duplication on the power consumption, we add a set of registers on the inputs of each bit-width region and we perform clock gating to avoid the switching of operands not involved in the current SIMD operation.
%
Despite the area overhead of 19.9\% with respect to the starting Dot-Product unit, this design choice does not increase the critical path of the system, avoiding to look at strategies that would consider pipelines in between the multiplication and the accumulation phases.
%
Pipeline registers would result in execution stalls when computing back-to-back operations, introducing a huge overhead to the QNN workload, where most of the compuation consits of Sum-of-Dot-Product operations.
%
Moreover the power consumption of the core is kept unaltered thanks to the power-aware design, as shown in Section \ref{sec:impl_results}.

%
To integrate the mac\&load instructions into the core, we extend the ex-stage of RI5CY with an additional small register file, namely Neural Network Register File (NN-RF), and we extend the Dotp-Unit to provide it with the capability of fetching one (m\&lv1) or both (m\&lv2) the \textit{dotp} operands from the NN-RF. On the same trail, we provide the NN-RF with a write port connected to the Load Store Unit (LSU) of the core, so that the registers can be updated with a new memory element. The micro-architecture proposed allows to execute this family of instructions in one clock cycle latency, when the pipeline is fully operative and no stalls occur on the LSU-memory interface.
%
The datapath of the mac\&load instructions is reported in Figure \ref{fig:ml_datapath}, where we distinguish with different colors the specific datapath of the m\&lv1 (in green) and the m\&lv2 (in red), while in black we report the common hardware blocks and wires. %With the presented datapath, the mac\&load instructions execute in only one cycle.
%

As visible, in the m\&lv2 the NN-RF accepts 5-bit of Immediate from the ID-stage to control the registers and to handle their updating procedure, as described in Section \ref{sec:ISA}. Also, the Dotp-Unit is fed with both the operands coming from the NN-RF, while in the m\&lv1 the second operand is fetched from the GP-RF (``rs2'' in Figure). To this purpose, the NN-RF, in the m\&lv2 version, has an additional read port, named ``activation`` port to ease the discussion withouth loss of generality.
%
In both cases (m\&lv1 and m\&lv2) the ``rs1'' contains the address for the next memory access. It is sent to the LSU, which fetches from the memory the new data accordingly to the address, and stores it into the NN-RF (which features a single write port). The address then, is automatically incremented by one word using the ALU unit, like in the load with post-increment of the \textit{XpulpV2} ISA, and stored back using the additional write port available in the RI5CY general purpose register file (GP-RF). Since only one GP-RF write per cycle is admitted, we delay the storage of the Dotp-Unit result by one cycle. This will not impact the performance as we provide a forwarding method to solve eventual back-to-back dependencies on the Dotp-Unit output.
%
The hardware cost to support the mac\&load instructions is limited to a bunch of registers of the NN-RF and few interconnections and blocks within the ex-stage of the pipeline. As a consequence the impact of the design on the timing of the core is negligible. In addition, to avoid useless switching activities we perform operand isolation on the mac\&load operands at a cost of only few gates.

To assess the benefits of the mac\&load instructions at the micro-architecture level, we run simulations of the extended core executing \textit{MatMul} kernels, and considering the SIMD operations only, the m\&lv1, the m\&lv2 and the m\&lv2 with the optimized kernel layout. The outcome of this analysis is reported in Figure \ref{fig:OPEF_1core} in terms of cycles needed to perform a SIMD MAC operation (meaning that one \textit{dotp} 8-bit operation counts as one MAC).
%
As visible, the m\&lv1 improves the efficiency by 1.39 $\times$ with respect to the SIMD only case. Thanks to the enhanced m\&lv2 instruction, after initializing the NN-RF registers, the innermost loop of the \textit{MatMul} runs 1.10 $\times$ faster than the previous case. The optmized layout, possible only by exploiting the m\&lv2 instruction, brings an additional 1.07 $\times$ improvement, with a final efficiency of 1.08 cyc/MAC in the best case.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             CLUSTER INTEGRATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cluster integration}
\label{sec:clust_integration}
% OPEF MULTICORE
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/ML_multicore_opef_2.pdf}
    \caption{MAC Operation Efficiency of the PULP cluster on 8-bit Matrix Multiplication (\textit{MatMul}) kernels.}
    \label{fig:opef_multicore}
\end{figure}

After evaluating the improvement of the \textit{XpulpNN} ISA on a single-core execution of the \textit{MatMul} kernel, we integrate the extended RI5CY core into a PULP cluster of eight processors.
%
Since the QNN workload is highly parallelizable, we expect a near-linear scaling of the performance when moving from single- to multi-core contexts \cite{garofalo2020pulp}. 
%
We report in Figure \ref{fig:opef_multicore} the results of the execution of the 8-bit \textit{MatMul} kernel in terms of cycle needed by each core to execute a SIMD MAC operation, considering the execution of the kernel first with the m\&lv1 and then with the m\&lv2 instruction.
%
The analysis carried out shows some drawbacks of the m\&lv1 instruction that limits the efficiency of the computation in a multi-core context.
%
As visible from Figure \ref{fig:opef_multicore}, when executing the \textit{MatMul} kernel with m\&lv1 on eight cores, its efficiency decreases with respect to the single core execution. As described in Section \ref{sec:microarchi}, the m\&lv1 generates non-negligible traffic on the core-memory interface. In a multi-core context this traffic translates in many TCDM contentions, causing each core to wait for the data from the memory more than one cycle. 
%
If we split the L1 memory over more banks we are able to partially limit this effect. More in detail, if we consider a banking factor of four (``BF4'') (i.e. we double the baseline banking factor of two) the efficiency of the computation on eight cores increases by $5\%$, almost reaching the ones of the single core. However such a choice has non-negligible impact on the power consumption of the system.
%
Instead, the m\&lv2 seems not to suffer from this limitation, thanks to its capability to keep in the NN-RF one operand as long as we need, reducing the traffic on the core-memory interface when not needed.
%
In a baseline configuration of the cluster (i.e. banking factor 2) the m\&lv2 reaches almost the same efficiency as in the ``BF4'' configuration. 




==> text/06_discussion.tex <==
\section{Discussion}

==> text/table_power_area.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[t]
\label{tab:area_power}
\begin{tabular}{@{}ccccclllllllllllllllllllll@{}}
\cmidrule(r){1-5}
\multicolumn{5}{|c|}{\textbf{Area {[}um2{]} (Overhead vs. baseline {[}\%{]})}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textbf{RI5CY}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ext. RI5CY\\ (without m\&l)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ext. RI5CY\\ (with m\&lv1)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ext. RI5CY\\ (with m\&lv2)\end{tabular}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Total Cluster}} & \multicolumn{1}{c|}{970856} & \multicolumn{1}{c|}{982310 ( 1.1 \% )} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{1011254 (4.1 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Tot. Cluster\\ (32 tcdm banks)\end{tabular}}} & \multicolumn{1}{c|}{995210} & \multicolumn{1}{c|}{1030945 (3.6 \%)} & \multicolumn{1}{c|}{1026194 (3.11 \%)} & \multicolumn{1}{c|}{1053446 ( 5.9 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Total Core}} & \multicolumn{1}{c|}{35131} & \multicolumn{1}{c|}{39589 (12.7 \%)} & \multicolumn{1}{c|}{41492 (18 \%)} & \multicolumn{1}{c|}{41296 (17.5 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{EX-Stage}} & \multicolumn{1}{c|}{13385} & \multicolumn{1}{c|}{15836 (18.3 \%)} & \multicolumn{1}{c|}{17515 (30.9 \%)} & \multicolumn{1}{c|}{17744 (32.6 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{5}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Power Consumption of the COREs {[}mW{]}\\ on a 8-bit MatMul, 0.65V, 200MHz (SIMD used)\end{tabular}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Leak. Power}} & \multicolumn{1}{c|}{0.053} & \multicolumn{1}{c|}{0.055} & \multicolumn{1}{c|}{0.057} & \multicolumn{1}{c|}{0.063} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Dyn. Power}} & \multicolumn{1}{c|}{0.512} & \multicolumn{1}{c|}{0.538} & \multicolumn{1}{c|}{0.0557} & \multicolumn{1}{c|}{0.568} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Tot. Power}} & \multicolumn{1}{c|}{0.565} & \multicolumn{1}{c|}{0.593 (5 \%)} & \multicolumn{1}{c|}{0.614 ( 9\%)} & \multicolumn{1}{c|}{0.631 (11.7 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{5}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Power Consumption of the COREs {[}mW{]}\\ on a GP Application, 0.65V, 200MHz\end{tabular}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Leak. Power}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Dyn. Power}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{Tot. Power}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{5}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Total Power Consumption of the PULP cluster {[}mW{]}, \\ 0.65V, 200MHz\\ (Overhead vs baseline {[}5{]})\\ \{Overhead vs SIMD only {[}\%{]}\}\end{tabular}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{MatMul 32-bit}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{MatMul 8-bit}} & \multicolumn{1}{c|}{8.85} & \multicolumn{1}{c|}{8.94 (1 \%)} & \multicolumn{1}{c|}{9.18 (3.7 \%) \{2.7 \%\}} & \multicolumn{1}{c|}{9.24 (4.4\%)\{3.3\%\}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{(with m\&lv2)}} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{10.8 (22 \%)\{20.8 \%\}} & \multicolumn{1}{c|}{10.2 (15.2\%)\{14.1\%\}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{MatMul 4-bit}} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{8.53} & \multicolumn{1}{c|}{8,73 \{2.3 \%\}} & \multicolumn{1}{c|}{8.82 \{2.2\%\}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{(with m\&lv2)}} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{9.95 \{16.6 \%\}} & \multicolumn{1}{c|}{10.1 \{19.3 \%\}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{MatMul 2-bit}} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{9.04} & \multicolumn{1}{c|}{9.28 \{2.7 \%\}} & \multicolumn{1}{c|}{9.26 \{2.4 \%\}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{(with m\&lv2)}} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{--} & \multicolumn{1}{c|}{11.2 \{23.4 \%\}} & \multicolumn{1}{c|}{10.8 (19.4\%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{|c|}{\textbf{GP Application}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cmidrule(r){1-5}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \bottomrule
\end{tabular}
\caption{Area and Power Consumption of our solution compared to the baseline RI5CY core.}
\end{table*}\textbf{}

==> text/table_power_area_v2.tex <==
\begin{table}[t]
\caption{Area and Power Consumption Results. Corner TT: TT, 400 MHz, 0.65V. Corner SS: SS, 200 MHz, 0.59V.}
\label{tab:area_power}
\centering

\begin{tabular}{lcccc}

\hline \hline
& \multicolumn{2}{|c|}{} &  \multicolumn{2}{|c}{} \\
 & \multicolumn{2}{|c|}{\textbf{RI5CY}} & \multicolumn{2}{|c}{\textbf{Ext. RI5CY }} \\
 &\multicolumn{2}{|c|}{(baseline)} & \multicolumn{2}{|c}{\textbf{(with m\&lv2)}}  \\ \hline \hline \\
 
 
 %%%%% AREA
 \multicolumn{5}{c}{\textbf{Area {[}um2{]} (Overhead vs. baseline {[}\%{]})}} \\ \hline 
 
 \textbf{Tot. Cluster} & \multicolumn{2}{|c|}{970856} & \multicolumn{2}{|c}{1011254 \textbf{(4.1 \%)}} \\ \hline
 
\textbf{Tot. Cluster } & \multicolumn{2}{|c|}{995210} & \multicolumn{2}{|c}{1053446 \textbf{( 5.9 \%)}} \\
\textbf{(32 tcdm banks)} & \multicolumn{2}{|c|}{} & \multicolumn{2}{|c}{} \\ \hline

\textbf{Total Core} & \multicolumn{2}{|c|}{35131} & \multicolumn{2}{|c}{41296 \textbf{(17.5 \%)}} \\ \hline

\textbf{EX-Stage} & \multicolumn{2}{|c|}{13385} & \multicolumn{2}{|c}{17744 (32.6 \%)} \\ \hline \hline \\


%%%%% FREQUENCY
\multicolumn{5}{c}{\textbf{Maximum Frequency {[}MHz{]}}} \\ \hline
%%%% CORNERS
\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \textbf{Slow} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \multicolumn{1}{|c}{\textbf{Slow}} \\ \hline
\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{400 } & 200 & \multicolumn{1}{|c|}{400 } & 200 \\ \hline \hline \\ 


%%%%% POWER CONSUMPTION CORE
\multicolumn{5}{c}{\textbf{Average Power Consumption of the CORE {[}mW{]}}}  \\ 
\multicolumn{5}{c}{ \textbf{on an 8-b MatMul (Overhead vs. baseline {[}\%{]}}} \\ \hline
%%%% CORNERS
\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \textbf{Slow} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \multicolumn{1}{|c}{\textbf{Slow}} \\ \hline
%%% VALUES
\multicolumn{1}{c|}{\textbf{Leak. Power}} & \multicolumn{1}{|c|}{0.108} & \multicolumn{1}{|c|}{0.055} & 0.122 & \multicolumn{1}{|c}{0.063}\\
\multicolumn{1}{c|}{\textbf{Dyn. Power}} & \multicolumn{1}{|c|}{1.78} & \multicolumn{1}{|c|}{0.577} & 1.82 & \multicolumn{1}{|c}{0.588}  \\
\multicolumn{1}{c|}{\textbf{Tot. Power}} & \multicolumn{1}{|c|}{1.89} & \multicolumn{1}{|c|}{0.632} & 1.95 \textbf{(3.17\%)} & \multicolumn{1}{|c}{0.651 \textbf{(3\%)}}  \\ \hline \hline \\

%%%%% POWER CONSUMPTION CORE GP APP
\multicolumn{5}{c}{\textbf{Average Power Consumption of the CORE {[}mW{]}}}  \\ 
\multicolumn{5}{c}{ \textbf{on a GP-application (Overhead vs. baseline {[}\%{]}}} \\ \hline 
%%%% CORNERS
\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \textbf{Slow} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \multicolumn{1}{|c}{\textbf{Slow}} \\ \hline
%%% VALUES
\multicolumn{1}{c|}{\textbf{Leak. Power}} &  &&& \\
\multicolumn{1}{c|}{\textbf{Dyn. Power}}&  &&& \\ 
\multicolumn{1}{c|}{\textbf{Dyn. Power}}&  &&& \\ \hline \hline \\


%%%%% POWER CONSUMPTION CLUSTER
\multicolumn{5}{c}{\textbf{Total Power Consumption of the PULP cluster {[}mW{]}}} \\ 
\multicolumn{5}{c}{\textbf{(Overhead vs baseline {[}\%{]})} }\\ \hline
%%%% CORNERS
\multicolumn{1}{c|}{} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \textbf{Slow} & \multicolumn{1}{|c|}{\textbf{Typ.}} & \multicolumn{1}{|c}{\textbf{Slow}} \\ \hline


\multicolumn{1}{c|}{\textbf{MatMul 32-bit}} & & \multicolumn{1}{|c|}{}& & \multicolumn{1}{|c}{}\\ \hline
\multicolumn{1}{c|}{\textbf{MatMul 8-bit}} & 26.1 & \multicolumn{1}{|c|}{9.22} & 26.1 & \multicolumn{1}{|c}{9.24 (0.2 \%)} \\ \hline
\multicolumn{1}{c|}{\textbf{(with m\&lv2)} }& -- & \multicolumn{1}{|c|}{--} & 27.3 (4.7 \%) & \multicolumn{1}{|c}{10.2 (14\%)}\\ \hline
\multicolumn{1}{c|}{\textbf{MatMul 4-bit}} & -- & \multicolumn{1}{|c|}{--} & 24.4 & \multicolumn{1}{|c}{8.82} \\ \hline
\multicolumn{1}{c|}{\textbf{(with m\&lv2)}} & -- & \multicolumn{1}{|c|}{--} & 25.8 & \multicolumn{1}{|c}{10.1} \\ \hline
\multicolumn{1}{c|}{\textbf{MatMul 2-bit}} & -- & \multicolumn{1}{|c|}{--} & 26.8 & \multicolumn{1}{|c}{9.26} \\ \hline
\multicolumn{1}{c|}{\textbf{(with m\&lv2)}} & -- & \multicolumn{1}{|c|}{--} & 28.2 & \multicolumn{1}{|c}{10.8}\\ \hline
\multicolumn{1}{c|}{\textbf{GP Application}} & & \multicolumn{1}{|c|}{}& &\multicolumn{1}{|c}{}\\ \hline






\end{tabular}

\end{table}

==> text/temp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Area and Power Consumption Results.}
\label{tab:my-table}
\begin{tabular}{cccccccccccccccccccccccccccccccc}
\multicolumn{5}{c}{\textbf{Area {[}um2{]} (Overhead vs. baseline {[}\%{]})}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textbf{RI5CY} &  & \textbf{\begin{tabular}[c]{@{}c@{}}Ext. RI5CY\\ (with m\&lv2)\end{tabular}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\



\multicolumn{5}{c}{\textbf{Area {[}um2{]} (Overhead vs. baseline {[}\%{]})}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Total Cluster} & \multicolumn{2}{c}{970856} & \multicolumn{2}{c}{1011254 (4.1 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{\begin{tabular}[c]{@{}c@{}}Tot. Cluster\\ (32 tcdm banks)\end{tabular}} & \multicolumn{2}{c}{995210} & \multicolumn{2}{c}{1053446 ( 5.9 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Total Core} & \multicolumn{2}{c}{35131} & \multicolumn{2}{c}{41296 (17.5 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{EX-Stage} & \multicolumn{2}{c}{13385} & \multicolumn{2}{c}{17744 (32.6 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\


\multicolumn{5}{c}{\textbf{Maximum Frequency {[}MHz{]}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{400 MHz} & 200 MHz & \multicolumn{1}{l}{400 MHz} & 200 MHz &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\


\multicolumn{5}{c}{\textbf{Average Power Consumption of the CORE {[}mW{]} on an 8-b MatMul (Overhead vs. baseline {[}\%{]}}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Leak. Power} & 0.108 & \multicolumn{1}{c}{0.055} & 0.122 & \multicolumn{1}{c}{0.063} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Dyn. Power} & 1.78 & \multicolumn{1}{c}{0.577} & 1.82 & \multicolumn{1}{c}{0.588} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Tot. Power} & 1.89 & \multicolumn{1}{c}{0.632} & 1.95 ( 3.17 \%) & \multicolumn{1}{c}{0.651 (3 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{5}{c}{\textbf{Average Power Consumption of the CORE {[}mW{]} on GP-app (Overhead vs. baseline {[}\%{]})}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Leak. Power} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Dyn. Power} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{Tot. Power} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{5}{c}{\textbf{Total Power Consumption of the PULP cluster {[}mW{]} (Overhead vs baseline {[}\%{]})}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} & \multicolumn{1}{l}{\textbf{TT,400MHz, 0.65V}} & \textbf{SS, 200MHz, 0.59V} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{MatMul 32-bit} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{MatMul 8-bit} & 26.1 & \multicolumn{1}{c}{9.22} & 26.1 & \multicolumn{1}{c}{9.24 (0.2 \%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{(with m\&lv2)} & -- & \multicolumn{1}{c}{--} & 27.3 (4.7 \%) & \multicolumn{1}{c}{10.2 (14\%)} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{MatMul 4-bit} & -- & \multicolumn{1}{c}{--} & 24.4 & \multicolumn{1}{c}{8.82} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{(with m\&lv2)} & -- & \multicolumn{1}{c}{--} & 25.8 & \multicolumn{1}{c}{10.1} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{MatMul 2-bit} & -- & \multicolumn{1}{c}{--} & 26.8 & \multicolumn{1}{c}{9.26} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{(with m\&lv2)} & -- & \multicolumn{1}{c}{--} & 28.2 & \multicolumn{1}{c}{10.8} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\textbf{GP Application} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-2} \cline{4-4} \cline{6-26}
\end{tabular}   
\end{table
